The EBLM project X. Benchmark masses, radii and temperatures for two fully convective M-dwarfs using K2

M-dwarfs are the most abundant stars in the galaxy and popular targets for exoplanet searches. However, their intrinsic faintness and complex spectra inhibit precise characterisation. We only know of dozens of M-dwarfs with fundamental parameters of mass, radius and effective temperature characterised to better than a few per cent. Eclipsing binaries remain the most robust means of stellar characterisation. Here we present two targets from the Eclipsing Binary Low Mass (EBLM) survey that were observed with K2: EBLM J0055-00 and EBLM J2217-04. Combined with HARPS and CORALIE spectroscopy, we measure M-dwarf masses with precisions better than 5%, radii better than 3% and effective temperatures on order 1%. However, our fits require invoking a model to derive parameters for the primary star. By investigating three popular models, we determine that the model uncertainty is of similar magnitude to the statistical uncertainty in the model fits. Therefore, whilst these can be considered benchmark M-dwarfs, we caution the community to consider model uncertainty when pushing the limits of precise stellar characterisation.

==> fitting_text_backup.tex <==

\subsection{Combined radial velocity and photometric modelling}


\iffalse
K2 photometry was modelled jointly with radial velocity measurements to determine the final orbital solution.  We performed a $\chi^2$ fit in a Bayesian framework to estimate the PPD of each parameter in the vector model. The vector model of parameters includes photometric zero-points for each $i^{th}$ light-curve --$zp_i$, $R_{\star}/a$, $k$, the impact parameter --$b = a\cos(i_{\rm orb})/R_{\star}$ where $i_{\rm orb}$ is the orbital inclination, the transit epoch --$\rm T_0$, the orbital period --$P$, the semi-amplitude of radial velocity measurements --$K$, the systematic radial velocity -- $\gamma$ and the change in systematic radial velocity with time --$d(\gamma)/dt$. Instead of fitting the argument of the periastron ($\omega$) and the eccentricity ($e$), we choose to use  $f_c = \sqrt{e} \cos \omega$ and  $f_s = \sqrt{e} \sin \omega$  since these have a uniform prior probability distribution and are not strongly correlated with each other. We also include a jitter term  ($\sigma_J$) to account for spot activity which can introduce noise in to the radial velocity measurements \citep{2006ApJ...642..505F}.

We used a custom binary star model to determine the best orbital solution. Our model used the method described by \citet{2016A26A...591A.111M} to solve Kepler's equations. The true anomaly, $\nu_i$, corresponding to time $t_i$ was used to calculate a radial velocity model for the primary component,
%
\begin{equation}\label{radial_velocity}
    V_{\rm 1} = K_1 \left( e \cos \omega + \cos \nu_i + \omega \right) + \gamma + (t_i - T_0)d(\gamma)/dt. 
\end{equation}
%
The projected separation between the primary and secondary components,
%
\begin{equation}\label{sky_projected_seperation}
\delta = \frac{1 - e^2}{1 + e \cos \nu_1} \sqrt{1 - \sin^2i_{\rm orb} \sin^2(\nu + \omega)},
\end{equation}
%
was used to model primary eclipses and the secondary eclipse of J0055$-$00. For primary eclipses, we used the analytical approximation presented by \citet{2019A&A...622A..33M} to describe an object eclipsing a star with limb-darkening described by the power-2 law. We fitted the decorrelated limb-darkening parameters suggested by \citet{2018A&A...616A..39M}, 
%
\begin{eqnarray}
&h_1 &= 1 - c(1 - 2^{-\alpha}),\\
&h_2 &= c2^{-\alpha},
\end{eqnarray}
%
where $c$ and $\alpha$ describe the intensity ($I$) across the surface of the primary star as a function of $\mu = \cos \gamma$, where $\gamma$ is the angle between a line normal to the stellar surface and the line of sight of the observer,
%
\begin{equation}
    I_\mu = 1 - c(1 - \mu^\alpha).
\end{equation}
%
We observed secondary eclipses for each system which permitted a measurement of the luminosity ratio between the primary and secondary component. The shape of the secondary eclipse is typically parameterised by the surface brightness ratio, $S = k^2 F_{\lambda,2} / F_{\lambda,\star}$, where $F_{\lambda}$ is the flux of each star observed in some bandpass. We assume the M-dwarf is uniformly illuminated where the normalised depth of a secondary eclipse is then given by $1-S \times k^2$. The primary eclipse was diluted was diluted by a factor of $k^2 (1 - F_{\lambda,2} / F_{\lambda,\star}$, although \citet{2019arXiv190412695G} found this effect to be less to be less than 500\,ppm for the earliest M-dwarfs in red transmission filters.  
\fi

\begin{table}[]
    \centering
        \caption{Parameters and priors (if any) used determine the orbital solution. Priors take the form of $\mathcal{U}(x,y)$ where $x$ and $y$ are the lower and upper limits of a uniform prior respectively and $\mathcal{G}(x,y)$ where $x$ and $y$ are the centre and width of a Gaussian prior. }
    \begin{tabular}{ccc}
    \hline
    \hline
       & parameter & prior \\ 
       \hline
       radial velocity & $T_0 / \rm day$ & - \\
                       & $P_{\rm orb} / \rm day$ & - \\
                       & $K_1 / \rm km\, \rm s^{-1}$ & $\mathcal{U}$(0, none)  \\
                       & $f_{\rm s}$ & $\mathcal{U}$($-0.5$, 0.5)  \\
                       & $f_{\rm c}$ & $\mathcal{U}$($-0.5$, 0.5)  \\
                       & $\gamma / \rm km\, \rm s^{-1}$  &  -  \\
                       & $\dot{\gamma} / \rm km\, \rm s^{-1}\, \rm yr^{-1}$ &  $\mathcal{U}$($-1$, 1)  \\
                       & $\sigma_{\rm RV}/ \rm km\, \rm s^{-1}$ & $\mathcal{U}$(0, none)  \\
       \hline
       light curve  & $R_\star / a$ & $\mathcal{U}$(0, 0.5) \\
                    & $R_2 / R_\star$ & $\mathcal{U}$(0, 0.5) \\
                    & $b$ & $\mathcal{U}$(0, 1+$k$) \\
                    & $h_1$ & $\mathcal{G}$(0, 1+$k$) \\
                    & $h_2$ & $\mathcal{G}$(0, 1+$k$) \\
                    & $S$   & $\mathcal{U}$(0, 0.5) \\
                    & $z_p$ & - \\
       \hline 
       \textsc{celerite} & $\ln(B/ \rm mmag^2)$ & $\mathcal{U}$($-13$, $-9$) \\
              & $\ln(L/ \rm day)$ & $\mathcal{U}$(0.5,8.) \\
              & $\ln(P_{\rm rot}/ \rm day)$ & $\mathcal{U}$(0.7,8.0) \\
              & $\ln(C)$ & $\mathcal{U}$(-5.0,8.0) \\
              & $\ln(\sigma/ \rm mmag)$ & $\mathcal{U}$(-5.0,8.0) \\
        \hline
    \end{tabular}
    \label{table_2:parameters}
\end{table}

\iffalse
To generate a red-noise model, we use the \textsc{celerite} package \citep{2017AJ....154..220F}. We followed the example detailed in Section 6.5 from \citet{2017AJ....154..220F} to model quasi-periodic variations in exoplanet lightcurves. We constructed a \textsc{celerite} co-variance function,
%
\begin{equation}
    k(\tau) = \frac{B}{2+C}e^{-\tau/L} \left[ \cos \left( \frac{2 \pi \tau}{P_{\rm rot}} \right) + (1 + C) \right] + \sigma^2,
\end{equation}
%
where $B>0$, $C>0$, and $L>0$. Here, $\tau_k$ is the time difference between two observations, $B$ is the amplitude of quasi-period variations, $L$ describes their respective timescales, $P_{\rm rot}$  is the rotational period of the primary star, $C$ is an arbitrary factor, and $\sigma$ is an additional jitter term to account for additional uncertainty in photometric measurements. Similar to the example in Section 6.5 from \citet{2017AJ....154..220F}, we fit the logarithm of each parameter along with uniform priors.

The parameters we fitted along with respective priors can be found in Table \ref{table_2:parameters}. We compare models to data in a Bayesian framework with a log-likelihood function $\mathcal{L} = \exp(-\chi^2/2)$, with
%
\begin{equation}
    \chi^2 = \sum_i \frac{(m_{\rm i} - m_{\rm model})^2}{\sigma_{m_{\rm  i}}^2 + \sigma_{\rm LC}^2} + \sum_i \frac{(rv_{\rm i} - rv_{\rm model})^2}{\sigma_{rv_{\rm i}}^2 + \sigma_{\rm RV}^2}
\end{equation}
%
Here, $m_{\rm i}$ and $rv_{\rm i}$ represent the $i^{\rm the}$ measurement of magnitude and radial velocity with standard errors $\sigma_{\rm m_i}$ $\sigma_{\rm rv_i}$, respectively. We initiated 50 walkers and generated 20,000 draws, after an initial burn-in phase of 50,000 draws using \textsc{emcee}. We selected the trial step with the highest value of $\mathcal{L}$ as the measurement for each parameter.  The uncertainties were calculated from the largest difference between the median and the $16^{th}$ and $84^{th}$ percentile of the cumulative PPD for each parameter from the second chain.

\fi


\subsection{Flattening \ktwo\ and \tess\ photometry}

\ktwo photometry is sufficiently precise that we can clearly identify  primary and secondary eclipses. We performed a preliminary fit for each object to determine the best fitting transit model and corresponding contact points for both primary and secondary eclipses. Data within these contact points were masked and a Savitzky–Golay filter with a size of 103 data points ($\sim$2.5 days) and polynomial order 3 to encapsulate the out-of-transit trend. 


\subsection{Moddeling}

We used the binary star model described by \citet{2020MNRAS.491.1548G} to assess models of radial velocity and transit photometery. This uses the analytical transit model \textsc{qpower-2} presented by \citet{2019A&A...622A..33M} which assumes stars are limb-darkened by the power-2 law. We fit decorrelated limb-darkening parameters $h_1$ \& $h_2$ (from Eqn. 1 \& 2 of \citealt{2018A&A...616A..39M}) with Gaussian priors centred on values interpolated from Table\,2 of \citet{2018A&A...616A..39M} and widths of 0.003 and 0.046 respectively. The \kepler\ and \wasp\ transmission throughputs are sufficiently different that we fit independent values of $h_1$ and $h_2$ for each dataset.

Our model vector included the transit epoch, $T_0$, the orbital period, $P$, $R_1 / a$, $k=R_2/R_1$, $b$, independent values of the photometric zero-point, $zp$, $h_1$ and $h_2$ for each filter, the surface brightness ratio, $SBR$, the semi-amplitude, $K_1$, and the systematic radial velocity of the primary star, $\gamma$. Instead of fitting the argument of the periastron ($\omega$) and the eccentricity ($e$), we used  $f_c = \sqrt{e} \cos \omega$ and  $f_s = \sqrt{e} \sin \omega$ since these have a uniform prior probability distribution and are not strongly correlated with each other. For \wasp datasets, we include a jitter term, $J$, added in quadrature to photometric uncertainties to account for various stellar effects and non-optimal observing conditions. 










We also include a jitter term added in quadrature to radial velocity uncertainties ($J$) to account for spot activity, pulsations, and granulation which can introduce noise in to the radial velocity measurements \citep{2006ApJ...642..505F}. This was added in quadrature to the uncertainties associated with each RV measurement. We fit a similar term for each photometric data set, $\sigma$, which was also added in quadrature to photometric uncertainties. We assume a common third light contribution of 7.13\% in all transmission filters.

We used the ensemble Bayesian sampler \textsc{emcee} \citep{2013PASP..125..306F} to sample parameter space. We initiated 50 Markov chains and generated 100,000 trial steps, discarding the first 50,000 steps as part of the burn-in phase. We visually inspected each Markov chain to ensure convergence well before the 50,000$^{th}$ draw. The trial step with the highest log-likelihood was selected as our measurement for each fitted parameter. We adopted the difference between each measured parameter and the $16^{\rm th}$ and $84^{\rm th}$ percentiles of their cumulative posterior probability distributions as a measurement of asymmetric uncertainty. Fitted parameters are reported in Table\,\ref{tab:parameters} and shown in Fig.\,\ref{fig:Figure_3}.




\iffalse
\begin{table*}
\caption{The atmospheric parameters of 3 EBLMs discovered by the WASP survey.}              % title of Table
\label{EBLMs_atmos}      % is used to refer this table in the text
\centering   
\resizebox{0.9\linewidth}{!}{%                                   % used for centering table
\begin{tabular}{l c c c c c}          % centered columns (4 columns)

\hline                        % inserts double horizontal lines
 
 & J0055$-$00 
 & J0457$+$14 
 & J1652$-$19
 & J2217$-$04 \\
 
  
 & \object{EPIC220196587} 
 & \object{EPIC246712205}
 & \object{EPIC205148699}
 & \object{EPIC206500801}\\
 
\hline 

\multicolumn{3}{l}{From SED fitting} \\

$\rm T_{\rm eff, phot}$ (K)
& $5880 \pm 110$ (G1)
& $7385 \pm 228$ (A9)
& $6226 \pm 180$ (F7)
& $5810 \pm 120$ (G2)\\

$\rm E(B-V)$
& $0.031 \pm 0.023$
& $0.329 \pm 0.040$
& $0.285 \pm 0.033$
& $0.095 \pm 0.024$\\

$g'_0$
& $11.214 \pm 0.091$
& $11.076 \pm 0.126$
& $11.875 \pm 0.133$
& $12.283 \pm 0.121$\\
\\


\multicolumn{3}{l}{From spectroscopy} \\

$\rm T_{\rm eff}$ $\rm(K)$
& $5969 \pm 85$
& $7373 \pm 85$
& $6262 \pm 85$ 
& $5848 \pm 85$\\

$\log g$ (dex)  
& $4.36 \pm 0.13$ 
& $5.04 \pm 0.13$ 
& $4.56 \pm 0.13$ 
& $4.17 \pm 0.13$ \\


$\xi_{\rm t}\, (\rm km\,s^{-1})$
& $1.17 \pm 1.50$
& $1.92 \pm 1.50$
& $1.26 \pm 1.50$
& $1.15 \pm 1.50$ \\

$v_{\rm mac}\, (\rm km\,s^{-1})$
& $4.67 \pm 1.50$
& $19.51 \pm 1.50 $
& $6.84 \pm 1.50$
& $4.25 \pm 1.50$ \\

Vsin$i$ (km\,s$^{-1}$)
& $ \leq 5$
& $72 \pm 1$
& $11.56 \pm 1.35$ 
& $7.97 \pm 1.35$ \\



$\rm [Fe/H]$
& $0.39 \pm 0.06$
& $0.43 \pm 0.30$
& $0.18 \pm 0.06$
& $0.27 \pm 0.30$\\

$\log \rm A(Li) + 12$
& $2.5 \pm 0.1$ 
& - 
& - 
& -\\ \\
\hline

\hline                                             %inserts single line
\end{tabular}}
\end{table*}
\fi
